Static Analysis of Lockless Microcontroller C Programs

Concurrently accessing shared data without locking is usually a subject to race conditions resulting in inconsistent or corrupted data. However, there are programs operating correctly without locking by exploiting the atomicity of certain operations on a specific hardware. In this paper, we describe how to precisely analyze lockless microcontroller C programs with interrupts by taking the hardware architecture into account. We evaluate this technique in an octagon-based value range analysis using access-based localization to increase efficiency.

==> eptcsdata.tex <==
\providecommand{\firstpage}{103}
\providecommand{\publicationstatus}{F. Cassez, R. Huuck, G. Klein and B. Schlich (eds.):\\ Systems Software Verification Conference 2012 (SSV 2012)\\
EPTCS 102, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.102.10}{10.4204/EPTCS.102.10}}
\pdfoutput=1

